Detection of Face Recognition Adversarial Attacks

Deep Learning methods have become state-of-the-art for solving tasks such as Face Recognition (FR). Unfortunately, despite their success, it has been pointed out that these learning models are exposed to adversarial inputs - images to which an imperceptible amount of noise for humans is added to maliciously fool a neural network - thus limiting their adoption in real-world applications. While it is true that an enormous effort has been spent in order to train robust models against this type of threat, adversarial detection techniques have recently started to draw attention within the scientific community. A detection approach has the advantage that it does not require to re-train any model, thus it can be added on top of any system. In this context, we present our work on adversarial samples detection in forensics mainly focused on detecting attacks against FR systems in which the learning model is typically used only as a features extractor. Thus, in these cases, train a more robust classifier might not be enough to defence a FR system. In this frame, the contribution of our work is four-fold: i) we tested our recently proposed adversarial detection approach against classifier attacks, i.e. adversarial samples crafted to fool a FR neural network acting as a classifier; ii) using a k-Nearest Neighbor (kNN) algorithm as a guidance, we generated deep features attacks against a FR system based on a DL model acting as features extractor, followed by a kNN which gives back the query identity based on features similarity; iii) we used the deep features attacks to fool a FR system on the 1:1 Face Verification task and we showed their superior effectiveness with respect to classifier attacks in fooling such type of system; iv) we used the detectors trained on classifier attacks to detect deep features attacks, thus showing that such approach is generalizable to different types of offensives.

==> sec/4_method.tex <==
\section{Adversarials Detection Method} \label{method}

\begin{figure*}[t]
\includegraphics[width=\textwidth]{images/deep_adversarial_detection_scheme.pdf}
\caption{Schematic view of the detection algorithm. The deep features are extracted at the end of each of the bottlenecks of the Se-ResNet-50 model.} \label{fig:detector_scheme}
\end{figure*}

The ultimate goal of our work was to detect adversarials samples.
In order to accomplish that, we started from the approach we exploited in~\cite{carrara2018adversarial}.
During the forward step of the threatened model, we collected the deep features, at the output of specific layers, to which we subsequently applied an average pooling operation, thus obtaining a single features vector at each selected layer.
Then, we computed the distance among each vector and the class representatives, centroids or medoids, of each class, at each layer, obtaining an embedding which represented the trajectory of the input image in the features space.
Such a trajectory was then fed to a binary classifier that is used as adversarial detector.\\
In our experiments, we used the test set of the VGGFace2~\citep{cao2018vggface2} dataset, which comprises 500 identities, and the state-of-the-art Se-ResNet-50 from~\cite{cao2018vggface2}.
Specifically, we extracted the deep features at the end of each of the 16 bottleneck blocks of the model.
As the adversarial detector, we tested two different architectures: a Multi Layer Perceptron (MLP) and a Long-Short Term Memory (LSTM) network.
The former was made by a hidden layer of 100 units followed by the ReLU non-linear function and a Dropout layer.
The latter had a hidden state size of 100.
In both cases, the output of the detector was fed into a Fully Connected (FC) layer followed by a sigmoid activation function.
A schematic view of the entire system is shown in \autoref{fig:detector_scheme}.
Considering the 16 bottlenecks of the model from which we collected the deep features and the 500 different identities of the dataset, each embedding was then represented by a 8000-dimensional vector.
In this vector, each \emph{i}-th dimension represented the distance between the \emph{i}-th internal representation and a class representative in a specific layer.

==> sec/5_experimental_results.tex <==
\section{Experimental Results} \label{experimental_results}

In this section, we reported the experimental results we have obtained so far.
First, we focused on the detection of the attacks against a state-of-the-art FR model acting as a classifier.
We crafted adversarial inputs by means of known algorithms, and then we trained and tested our detector against them.
Afterwards, we generated deep features (DF) attacks (\Cref{deep_representation_attack}) using a kNN algorithm as guidance for the optimization procedure.

The goal of this approach was to fool a FR system in which the CNN was only used as a features extractor, while the final identity was assigned according to the output of a similarity measurement among deep features.
In our experiments, we considered a system that used a kNN algorithm to assign an identity to the probe image.
This is a typical solution for FR systems to fulfill the Face Identification task. 
Thereafter, we used these deep adversarial features to attack a FR system against the Face Verification task. 
Finally, we used the detectors, trained on the classifier attacks, to detect deep features attacks thus showing the generalization property of the detection approach.\\
%\subsection{Dataset} \label{vggface2_dataset}
As we already stated, in our experiments we employed the test set of the VGGFace2~\citep{cao2018vggface2} dataset which comprises 500 identities, with an average of $\sim$340 images for each identity. 

As a first step, for each of the 500 classes of the dataset, we randomly selected 10 images to be used as ``natural" images and 10 to be used for adversarial synthesis.
These selected images were then used to train and test the adversarial detector.

We then split the remaining part of the dataset into train, validation and test sets and used them to train a FC layer on top of the state-of-the-art CNN we used in the study presented in \Cref{micsl_attack}.

\subsection{Classifier Attacks and Detection} \label{micsl_attack}
In the first set of experiments, we focused on the classifier attacks.
As a first step, we replaced the classifier layer of the state-of-the-art facial recognition model~\citep{cao2018vggface2} with a 500-ways FC layer, and we trained it.
To train the model, we used the SGD optimizer with batch size of 256 and a learning rate of $10^{-3}$ halved every time the loss plateaus.
As a preprocessing step, we resized the images so that the shortest side measured 256 pixels.
Afterwards, we randomly cropped a 224x224 region of the image, and we subtracted the average pixel value channel-wise.
For model evaluation, we used the same preprocessing with the exception that the random crop was substituted by a central crop. %The final model accuracy was 98.4\%.\\

In order to produce adversarial samples, we used the \emph{foolbox}\footnote{\url{https://foolbox.readthedocs.io/en/stable/}} implementation of the BIM~\citep{kurakin2016adversarial}, MI-FGSM~\citep{dong2018boosting}, and CW~\citep{carlini2017towards}, with $L_2$ norm, attacks.
As far as the first two are concerned, we considered a maximum perturbation $\epsilon \in \{0.03, 0.07, 0.1, 0.3\}$,
number of iterations $\in \{30, 50\}$, and for each combination, we considered the targeted and the untargeted versions of the attacks.
The $\epsilon$ values were considered as fractions with respect to the maximum pixel value, which was 255.
Instead, for the CW~\citep{carlini2017towards} attack, we considered the implemented default value of the parameters, i.e. 5 binary search steps and a number of max iterations equals to 1000.
After the adversarial samples generation, we trained the detectors.
The MLP and the LSTM were both trained using the Adam optimizer~\citep{kingma2014adam} for 150 epochs with a batch size of 256 and an initial learning rate ranging from $10^{-4}$ to $10^{-3}$ which was reduced by a factor 10 every time the loss reached a plateau.
Moreover, to balance the sample distribution within mini-batches, we employed a weighted random sampler thus avoiding a bias towards attacks with higher multiplicity.

In \autoref{fig:detector_rocs_aucs}, we showed the Receiving Operating Characteristics (ROC) curves from the adversarial detection considering targeted and untargeted attacks for each architecture, distance metric, and class representative combination.
As a summary, in \autoref{tab:table_auc_attack} we reported the Area Under the Curve (AUC) values relative to each attack considering their targeted and untargeted versions, respectively.

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth, height=6.cm]{images/rocs_2_targeted_untargeted.pdf}
\caption{ROCs for each model (LSTM or MLP), class repreentative (Centroids or Medoids), and distance metric ($L_2$ or cosine) combination. Left: targeted attacks. Right: untargeted attacks.} \label{fig:detector_rocs_aucs}
\end{figure*}

\begin{table*}[!h]
\caption{Area Under the Curve (AUC) values for each configuration of architecture, pivot-selection and embedding function considering each targeted and untargeted attack independently. The last column is a summary of the single-attacks AUCs.}
\label{tab:table_auc_attack}
{\setlength\doublerulesep{0.4pt} 
\begin{tabularx}{\textwidth}{l>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering}X>{\centering\arraybackslash}X}
\toprule[1pt]\midrule[0.5pt]
Configuration & \multicolumn{2}{c}{BIM} & \multicolumn{2}{c}{CW} & \multicolumn{2}{c}{MI-FGSM} & \multicolumn{2}{c}{Macro-AUC} \\
& Targ. & Untarg. & Targ. & Untarg. & Targ. & Untarg. &  Targ. & Untarg. \\
\hline

LSTM + M + $L_2$ &  0.977 & 0.878 & 0.871 & 0.615 & 0.986 & 0.889 & 0.944 & 0.794 \\
LSTM + C + $L_2$ &  0.970 & 0.863 & 0.857 & 0.596 & 0.982 & 0.869 & 0.936 & 0.776 \\
LSTM + M + cos   &  \textbf{0.986} & \textbf{0.929} & \textbf{0.904} & \textbf{0.599} & \textbf{0.991} & \textbf{0.930} &  \textbf{0.960} & \textbf{0.819} \\
LSTM + C + cos   &  0.968 & 0.884 & 0.895 & 0.568 & 0.981 & 0.886 & 0.948 & 0.779\\
MLP  + M + $L_2$ &  0.964 & 0.885 & 0.793 & 0.559 & 0.979 & 0.882 & 0.912 & 0.775\\
MLP  + C + $L_2$ &  0.962 & 0.874 & 0.808 & 0.557 & 0.979 & 0.874 & 0.916 & 0.768\\
MLP  + M + cos   &  0.890 & 0.763 & 0.668 & 0.460 & 0.940 & 0.769& 0.832 & 0.664 \\
MLP  + C + cos   &  0.868 & 0.730 & 0.720 & 0.467 & 0.915 & 0.739 & 0.834 & 0.645 \\

\midrule[0.5pt]\bottomrule[1pt]
\end{tabularx}
}
\end{table*}

% \begin{table*}[!h]
% \caption{Area Under the Curve (AUC) values for each configuration of architecture, pivot-selection and embedding function considering each targeted attack independently. The last column is a summary of the single-attacks AUCs.}
% \label{tab:table_auc_attack_targeted}
% {\setlength\doublerulesep{0.4pt} 
% \begin{tabularx}{\textwidth}{l>{\centering}X>{\centering}X>{\centering}X>{\centering\arraybackslash}X}
% \toprule[1pt]\midrule[0.5pt]
% Configuration & BIM & CW & MI-FGSM & Macro-AUC \\
% \hline
% LSTM + M + $L_2$ &  0.977 & 0.871 & 0.986 & 0.944 \\
% LSTM + C + $L_2$ &  0.970 & 0.857 & 0.982 & 0.936 \\
% LSTM + M + cos   &  \textbf{0.986} & \textbf{0.904} & \textbf{0.991} & \textbf{0.960} \\
% LSTM + C + cos   &  0.968 & 0.895 & 0.981 & 0.948 \\
% MLP  + M + $L_2$ &  0.964 & 0.793 & 0.979 & 0.912 \\
% MLP  + C + $L_2$ &  0.962 & 0.808 & 0.979 & 0.916 \\
% MLP  + M + cos   &  0.890 & 0.668 & 0.940 & 0.832 \\
% MLP  + C + cos   &  0.868 & 0.720 & 0.915 & 0.834 \\
% \midrule[0.5pt]\bottomrule[1pt]
% \end{tabularx}
% }
% \end{table*}

% \begin{table*}[!h]
% \caption{Area Under the Curve (AUC) values for each configuration of architecture, pivot-selection and embedding function considering each untargeted attack independently. The last column is a summary of the single-attacks AUCs.}
% \label{tab:table_auc_attack_untargeted}
% {\setlength\doublerulesep{0.4pt} 
% \begin{tabularx}{\textwidth}{l>{\centering}X>{\centering}X>{\centering}X>{\centering\arraybackslash}X}
% \toprule[1pt]\midrule[0.5pt]
% Configuration & BIM & CW & MI-FGSM & Macro-AUC \\
% \hline
% LSTM + M + $L_2$ & 0.878 & 0.615 & 0.889 & 0.794 \\
% LSTM + C + $L_2$ & 0.863 & 0.596 & 0.869 & 0.776 \\
% LSTM + M + cos   & \textbf{0.929} & \textbf{0.599}& \textbf{0.930} & \textbf{0.819} \\
% LSTM + C + cos   & 0.884 & 0.568 & 0.886 & 0.779 \\
% MLP  + M + $L_2$ & 0.885 & 0.559 & 0.882 & 0.775 \\
% MLP  + C + $L_2$ & 0.874 & 0.557 & 0.874 & 0.768 \\
% MLP  + M + cos   & 0.763 & 0.460 & 0.769 & 0.664 \\
% MLP  + C + cos   & 0.730 & 0.467 & 0.739 & 0.645  \\
% \midrule[0.5pt]\bottomrule[1pt]
% \end{tabularx}
% }
% \end{table*}

As it was made clear from \autoref{fig:detector_rocs_aucs} and \autoref{tab:table_auc_attack}, the LSTM with the medoids strategy gives the best results.
We can also notice how the CW~\citep{carlini2017towards} algorithm generates samples which are more difficult to be detected with respect to other algorithms. 
Moreover, it is clear how the untargeted attacks are typically more difficult to detect with respect to targeted attacks.
A possible explanation is that these attacks typically find the closest adversarial to the input image, thus an embedding method based on the distance between representation may have difficulties in detecting such attacks.
More details on this intuition were given in \Cref{deep_knn_attacks}.

% Finally, to visually understand the difference among the performances of the best detector on the various attacks, in \autoref{fig:best_detector_rocs_aucs}, we showed the relative ROCs.

% \begin{figure*}[t]
% \includegraphics[width=\textwidth]{images/rocs_best_model_targeted_untargeted.pdf}
% \caption{ROCs for each attack considering the best trained detector. Left: targeted attacks. Right: untargeted attacks.} \label{fig:best_detector_rocs_aucs}
% \end{figure*}

% According to \autoref{fig:best_detector_rocs_aucs}, it was made even clearer how hard it could be to detect adversarial samples generated by means of the CW~\cite{carlini2017towards} attack, especially considering untargeted attacks.

\subsection{Deep Features Attacks} \label{deep_knn_attacks}
As previously described in \Cref{deep_representation_attack}, it is possible to use the distance among deep representations as a guiding principle to craft adversarial samples instead of wrong label assignment.
Thus, nurturing this idea, we conducted new experiments in which we synthesized adversarial samples by using the distance among deep features as a guidance~\citep{sabour2015adversarial}.

The main idea behind this approach was to emulate a real world application scenario for a FR system in which a learning model is used as a features extractor whose output is used to fulfill the FR task by means of a similarity measurement.

\subsubsection{Face Identification} \label{face_identification}
As a real-world application case, we considered a system relying on a CNN and a kNN algorithm to accomplish the task of Face Identification.
Specifically, what typically happens in this case is that the features vector extracted from the probe face image has to be compared against a database of known identities to identify the person.
Each identity in the database is commonly represented by a template vector, i.e. a vector of features obtained by averaging several deep representations extracted from different images of the same person.
Subsequently, the similarity among the probe vector and the available templates is computed. 
This is what is required, for example, when testing FR model performances on the IJB-B~\citep{whitelam2017iarpa} and IJB-C~\citep{maze2018iarpa} benchmark datasets.
Following this principle, we evaluated the centroids for each of the 500 classes of the dataset.
To conduct our experiments, we used the original state-of-the-art model from~\citetp{cao2018vggface2} as a features extractor.

The adversarial generation was formulated as an optimization problem~\citep{sabour2015adversarial} solved by using the L-BFGS-B algorithm. Specifically, the constraint was used to set a threshold, $\delta$, on the maximum perturbation on each pixel of the original image as defined in \autoref{eq:deeprepr}.
In order to adapt the adversarial samples generation to our needs, we used a kNN classifier as guidance through the optimization procedure.
The optimization was then stopped once the targeted or untargeted attack's objective were met, that is, the kNN had classified the adversarial as belonging to the guide-image class or it had simply misclassified the face image considering targeted and untargeted attacks respectively. 
A schematic view of the algorithm is shown in \autoref{fig:deep_knn_sketch}.

\begin{figure*}[t]
\includegraphics[width=\textwidth]{images/deep_knn_sketch_2.pdf}
\caption{Schematic view of the adversarial generation procedure considering a state-of-the-art (SotA) model as features extractor and a kNN to asses the face identity. Left, before the attack. Right, after the attack.} \label{fig:deep_knn_sketch}
\end{figure*}

In our experiments we considered the values of $\delta \in \{5.0, 7.0, 10.0 \}$. An example of adversarial samples generated for each threshold value is shown in \autoref{fig:deep_examples}.

\begin{figure}[t]
\includegraphics[width=\linewidth]{images/deep_knn_example.pdf}
\caption{Adversarial samples for two different values of the threshold applied while solving the optimization problem. Top: $\delta=5.0$. Bottom: $\delta=10.0$} \label{fig:deep_examples}
\end{figure}

As we can see from \autoref{fig:deep_examples}, the generated images look equal to the original ones, i.e. there is not evident trace of the guide image into the adversarial one.
Considering targeted attacks we obtained a success rate of 95.6\%, 96.2\% and 96.3\% considering a value for $\delta = 5.0, 7.0, 10.0$, respectively. Instead, concerning untargeted attacks we obtained 96.8\% success rate for $\delta = 5.0, 7.0, 10.0$. 
%In all the samples generations we considered a maximum number of iterations equals to 700.

Differently from what was previously done in \Cref{micsl_attack}, we formulated our approach with the purpose of fooling a FR system which was not based on the simple model classification, but rather on similarities among deep representations. 
Indeed, it is not guaranteed that even if a model misclassifies a face image the adversarial deep representation will be then close enough to the representation of the wrong face class predicted by the model to fool the FR system.

In \autoref{fig:deep_feat_dist_break_down_t} we reported some results to justify our intuition.
The figure shows the distribution of the distance among the adversarial samples and the centroids of their relative classes considering classifier attacks (BIM~\citep{kurakin2016adversarialphysworld}, MI-FGSM~\citep{dong2018boosting}, and CW~\citep{carlini2017towards}) and DF attacks~\citep{sabour2015adversarial}, using a kNN as guidance. 

% \begin{figure}[!h]
% \includegraphics[width=\linewidth]{images/deep_feat_distances.pdf}
% \caption{Euclidean distance among deep features of adversarial samples and the assigned class centroid for classifier attacks (blue and orange) and kNN-guided attacks (green and red). `` - T" refers to targeted attacks while `` - UT" refers to untargeted attacks.} \label{fig:deep_feat_dist}
% \end{figure}

\begin{figure}[!h]
\includegraphics[width=\linewidth]{images/deep_feat_distances_divided_by_attack_targeted.pdf}
\caption{Euclidean distance among deep features of adversarial samples and the assigned class centroid considering each targeted attack singularly. The ``$\delta$" values correspond to the maximum $L_\infty$ perturbation allowed, for each pixel, for the kNN-guided attacks.} \label{fig:deep_feat_dist_break_down_t}
\end{figure}

% \begin{figure}[!h]
% \includegraphics[width=\linewidth]{images/deep_feat_distances_divided_by_attack_untargeted.pdf}
% \caption{Euclidean distance among deep features of adversarial samples and the assigned class centroid considering each untargeted attack singularly. The ``$\delta$" values correspond to the maximum $L_\infty$ perturbation allowed, for each pixel, for the kNN-guided attacks.} \label{fig:deep_feat_dist_break_down_ut}
% \end{figure}

As we can see from \autoref{fig:deep_feat_dist_break_down_t}, even though classifier attacks are able to fool a CNN model, the distance among them and the centroids of their classes is larger than the one obtained when considering malicious samples generated by means of the deep representation-based attack.
Thus, the latter represents a greater threat, with respect to the former types of attacks, for a FR system. We observed exactly the same behaviour for the untargeted attacks.
%Moreover, considering targeted and untargeted settings for the classifier attacks, the untargeted attacks are, on average, closer to the class centroids when compared to the targeted ones.
%This result supported the observation of the lower detection performance when we tested our detectors against untargeted attacks (\Cref{micsl_attack}).

Taking into account \autoref{fig:deep_feat_dist_break_down_t}, we can also notice that the average distance among the adversarial samples from its class centroid is quite stable among the three different values of the threshold we used when considering malicious images generated with the deep features attack.
This behaviour is supported by the observation that, independently from the threshold applied, the majority of the pixel perturbations are below, in the sense of an $L_\infty$ distance, a threshold of $5.0$.
Thus, a higher threshold has the effect that only a small portion of the image is perturbed above that threshold itself.
Specifically, considering the values of $\delta \in [5.0, 7.0, 10.0]$, the percentage of pixels whose perturbation is within an $L_\infty$ distance of 5.0 is 88.3\%, 85.6\%, 84.7\% respectively.
This behaviour is shown in \autoref{fig:deep_feat_mpp} for targeted attacks.
In the case of an untargeted setting, the results were almost identical.

\begin{figure}[!h]
\includegraphics[width=\linewidth]{images/deep_feat_mpp_untargeteg.pdf}
\caption{Maximum Pixel Perturbation (MPP) distribution considering targeted deep representations with different thresholds} \label{fig:deep_feat_mpp}
\end{figure}

\subsubsection{Face Verification} \label{face_verification}

In this section, we studied the ability of adversarial attacks to fool a FR system tested against the Face Verification protocol in which two face images are compared to claim if they belong to the same identity or not.
In the DL context, such decision is typically based upon similarity measurements among deep features extracted from the input faces. Specifically, once the model has been trained, the ROC curve is typically evaluated and a threshold value is chosen to be used as a reference value. Then, two faces are said to belong to the same identity if their similarity score exceeds the predefined threshold.
An example of a real world application scenario of this kind of protocol is a restricted access area control system.
Since in this type of applications the False Positives pose a greater threat than the False Negatives, it is important to evaluate the ROC curve down to very low values of the False Acceptance Rate (FAR). Such a demand translates into the requirement of evaluating the similarity scores among a larger number of negative pairs with respect to the positive ones.

Also in this case, the architecture of a FR system was made by a features extractor and a module which worked out the similarity measurements.
As a features extractor we used the state-of-the-art model from \citep{cao2018vggface2}, while we considered the cosine among features vectors as similarity measurement.

After the similarity evaluation, we obtained a ROC curve with an AUC value equals to 99.03\%. Then, we used the Equal Error Rate (EER) threshold which we found equal to 0.448 as a threshold value for the similarity measurement.
At this point, we hypothesized two possible scenarios for the adversarial attacks:

\begin{itemize}
    \item \emph{Impersonation Attack}. In this case, we wanted to fool the system by leading it to falsely predict that two face images belonged to the same identity.
    This situation emulated the case in which an intruder intends to enter a restricted area or, in a more general case, when someone is made recognizable as a different person.
    \item \emph{Evading Attack}. This case is the opposite of the previous one, i.e., we wanted the system not to recognize a person by saying that the two images belonged to different identities.
     This circumstance imitated the condition of someone whose identity is made unrecognizable.
\end{itemize}
From the FR system perspective, in the former case we needed the two images, which belonged to different people, to be ``equal enough", i.e., their similarity measurement had to be above the threshold we had previously defined, while in the latter case, we needed the two images to be ``distant enough", i.e. below the threshold.

To carry out these experiments, we considered the CW \citep{carlini2017towards} attack and the DF \citep{sabour2015adversarial} (kNN guided) one in the targeted and untargeted settings.
%What we expected was the deep representation attacks to be more effective with respect to the classifier attacks.
The results for the \emph{Impersonation Attack} scenario are reported in \Cref{fig:deep_adv_pred_same_targeted_untargeted}.
In this case, we considered what follows:
first, we randomly selected negative matches, and we kept the second image fix, i.e. we analysed pairs of faces $(x,\ x^{-})$ where $x^-$ was an image from a different class of $x$.
Then, we looked upon an adversarial image, whose adversarial class corresponded to the one of $x^-$, and used it in place of the first image of the match, i.e. we accounted the pairs $(x_{adv},\ x^{-})$ where $x_{adv}$ was an adversarial sample, crafted from $x$, whose adversarial class was the same as the $x^{-}$ one.
Then, we considered two similarity measurements: 
\begin{itemize}
    \item ``Original" which represents the value of the cosine among the deep features of $x$ and $x^-$;
    \item ``Adversarial" which represents the cosine between the deep features of $x_{adv}$ and $x^-$.
\end{itemize}

\begin{figure*}[!h]
\includegraphics[width=0.5\textwidth]{images/adv_pred_same_targeted.pdf}  
\includegraphics[width=0.5\textwidth]{images/adv_pred_same_untargeted.pdf}
\caption{Cosine similarity distribution for kNN-guided and CW attacks in the \emph{Impersonation Attack} scenario. Left: targeted attacks. Right: untargeted attacks. ``- Org" refers to the cosine among natural images while ``- Adv" refers to the cosine between the natural image and the adversarial one. The dash-pointed line represents the EER threshold.} \label{fig:deep_adv_pred_same_targeted_untargeted}
\end{figure*}

In \Cref{tab:pred_same_targeted_untargeted}, we reported the percentage of matches which overcame the EER threshold, before and after the attacks, considering the targeted and untargeted settings.

\begin{table}[!h]
\caption{Percentage of matches which overcame the EER threshold, before and after the attacks, considering the targeted and untargeted settings.}
\label{tab:pred_same_targeted_untargeted}
{\setlength\doublerulesep{0.4pt} 
\begin{tabularx}{0.5\textwidth}{l>{\centering}X>{\centering}X>{\centering}X>{\centering\arraybackslash}X}
\toprule[1pt]\midrule[0.5pt]
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Targeted}} & \multicolumn{2}{c}{\textbf{Untargeted}} \\ 
 & Original & Adv. & Original & Adv.  \\ \cline{2-5} 
$\delta=5$ & 4.0 & 92.8 & 19.9 & 81.5 \\ 
$\delta=7$ & 4.0 & \textbf{93.9} & 19.9 & \textbf{81.6} \\ 
$\delta=10$ & 4.4 & 93.6 & 19.8 & 81.1 \\ 
CW$^*$ & 50.5 & 34.9 & 8.0 & 9.3 \\ 
\midrule[0.5pt]\bottomrule[1pt]
\multicolumn{5}{@{}l}{$^*$  \cite{carlini2017towards}}
\end{tabularx}
}
\end{table}

As we can observe from \Cref{tab:pred_same_targeted_untargeted}, the DF attacks~\citep{sabour2015adversarial} (kNN-guided) are much more effective in pushing the similarity between the adversarials and the natural images above the recognition threshold.
Such conclusion holds for targeted and untargeted attacks.
Instead, the behaviour of the CW \citep{carlini2017towards} was unpredictable in this set up, thus we can conclude that even though the CW \citep{carlini2017towards} algorithm is among the strongest ones concerning classification attacks, it is not very effective against the Face Verification protocol. 

As far as the \emph{Evading Attack} scenario is concerned, the results are reported in \Cref{fig:deep_adv_pred_not_same_targeted_untargeted}.
Differently from the previous case, we started by collecting positive matches, i.e. pairs of images $(x,\ x^+)$ in which $x$ and $x^+$ belonged to the same class, and then we substituted $x$ with one of its adversarial, $x_{adv}$, whose class was different from the $x^+$ one.
Thus, we obtained the following similarity measurements:
 \begin{itemize}
    \item ``Original" which represents the value of the cosine among the deep features of $x$ and $x^+$;
    \item ``Adversarial" which represents the cosine between the deep features of $x_{adv}$ and $x^+$.
\end{itemize}
As we explained before, in this scenario the purpose of the attack was to push the similarity below the operational level of the FR system. 
% The difference with respect to the previous case is that while in the former the adversarial class and the natural image class were the same, in this case, the adversarial sample and the natural image belonged to different classes.

\begin{figure*}[!h]
\includegraphics[width=0.5\textwidth]{images/adv_pred_not_same_targeted.pdf} 
\includegraphics[width=0.5\textwidth]{images/adv_pred_not_same_untargeted.pdf}
\caption{Cosine similarity distribution for kNN-guided and CW attacks in the \emph{Evading Attack} scenario. Left: targeted attacks. Right: untargeted attacks. ``- Org" refers to the cosine among natural images while ``- Adv" refers to the cosine among the natural image and the adversarial one. The dash-pointed line represents the EER threshold.} \label{fig:deep_adv_pred_not_same_targeted_untargeted}
\end{figure*}

In \Cref{tab:pred_not_same_targeted_untargeted}, we reported the percentage of the matches that were below the EER threshold, before and after the attacks, considering the targeted and untargeted settings.

\begin{table}[!h]
\caption{Percentage of matches which are below the EER threshold, before and after the attacks, considering the targeted and untargeted settings.}
\label{tab:pred_not_same_targeted_untargeted}
{\setlength\doublerulesep{0.4pt}
\begin{tabularx}{0.5\textwidth}{l>{\centering}X>{\centering}X>{\centering}X>{\centering\arraybackslash}X}
\toprule[1pt]\midrule[0.5pt]
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Targeted}} & \multicolumn{2}{c}{\textbf{Untargeted}} \\ 
& Original & Adv. & Original & Adv.  \\ \cline{2-5}  
$\delta=5$ & 5.4 & 18.9 & 4.1 & 9.9 \\ 
$\delta=7$ & 4.3 & 22.9 & 4.3 & 11.4 \\ 
$\delta=10$ & 4.3 & \textbf{26.2} & 4.1 & \textbf{12.5} \\ 
CW$^*$ & 4.0 & 17.1 & 4.0 & 6.2 \\ 
\midrule[0.5pt]\bottomrule[1pt]
\multicolumn{5}{@{}l}{$^*$  \cite{carlini2017towards}}
\end{tabularx}
}
\end{table}

By observing \Cref{tab:pred_not_same_targeted_untargeted}, it was clear that the DF attacks~\citep{sabour2015adversarial} (kNN-guided) were more effective that the CW \citep{carlini2017towards} attacks in this case too.
We can noticed that on average the targeted attacks performed better than the untargeted ones, which was an expected behaviour since an untargeted attack ended as soon as the the adversarial is associated with a different identity, therefore it would not have gone any further from the original image.

\subsubsection{Detection}

Finally, we tested our detectors, trained on classifier attacks (\Cref{micsl_attack}), on the newly generated adversarial samples.
The resulting ROC curves, according to a threshold of $\delta=5$ and $\delta=10$ for targeted and untargeted attacks configurations, are shown in \autoref{fig:rocs_deep_repr_delta_5}.
We did not report the ROC for the case $\delta=7$ since the results were almost identical to the case with $\delta=10$.

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth,height=6.cm]{images/deep_adversarial_rocs_targeted_untargeted_thr_5_10.pdf}
\caption{ROCs for the best models considering adversarial attacks generated with $\delta=5.0$ (left) and $\delta=10.0$ (right). `` - T" refers to targeted attacks while `` - UT" refers to untargeted attacks.} \label{fig:rocs_deep_repr_delta_5}
\end{figure*}

As a summary, the AUC values were reported in \autoref{tab:tsb_deep_repr_t} for targeted and untargeted attacks.

\begin{table}[!h]
\caption{AUC values for the best performing detectors for each threshold value considered in our experiments for both targeted and untargeted attacks.}
\label{tab:tsb_deep_repr_t}
{\setlength\doublerulesep{0.4pt} 
\begin{tabularx}{\linewidth}{l>{\centering}X>{\centering}X>r}
\toprule[1pt]\midrule[0.5pt]
Configuration & \multicolumn{2}{c}{AUC} & $\delta$ \\
              &     Targ.    & Untarg.    &   \\
\hline
MLP  + $L_2$ & \textbf{0.976} & 0.492 & 5 \\
LSTM + cos   & 0.972 & 0.530 & 5 \\
LSTM + $L_2$ & 0.969 & \textbf{0.671} & 5 \\
MLP  + cos   & 0.915 & 0.571 & 5 \\ \hline
MLP  + $L_2$ & \textbf{0.977} & 0.481 & 7 \\
LSTM + cos   & 0.975 & 0.541 & 7 \\
LSTM + $L_2$ & 0.968 & \textbf{0.688} & 7 \\
MLP  + cos   & 0.908 & 0.596 & 7 \\ \hline
MLP  + $L_2$ & \textbf{0.980} & 0.467 & 10 \\ 
LSTM + cos   & 0.978 & 0.573 & 10 \\
LSTM + $L_2$ & 0.972 & \textbf{0.700} & 10 \\
MLP  + cos   & 0.915 & 0.609 & 10 \\
\midrule[0.5pt]\bottomrule[1pt]
\end{tabularx}
}
\end{table}
%
% \begin{table}[!h]
% \caption{AUC values for the best performing detectors for each threshold value considered in our experiments in the case of untargeted attacks.}
% \label{tab:tsb_deep_repr_ut}
% {\setlength\doublerulesep{0.4pt} 
% \begin{tabularx}{\linewidth}{l>{\centering}X>{\centering\arraybackslash}X}
% \toprule[1pt]\midrule[0.5pt]
% Configuration & AUC & $\delta$ \\
% \hline
% LSTM + cos   & 0.530 & 5 \\
% MLP  + $L_2$ & 0.492 & 5 \\
% MLP  + cos   & 0.571 & 5 \\
% LSTM + $L_2$ & \textbf{0.671} & 5 \\ \hline
% LSTM + cos   & 0.541 & 7 \\
% MLP + $L_2$ & 0.481 & 7 \\ 
% MLP  + cos   & 0.596 & 7 \\
% LSTM + $L_2$ & \textbf{0.688} & 7 \\ \hline
% LSTM + cos   & 0.573 & 10 \\
% MLP + $L_2$ & 0.467 & 10 \\
% MLP  + cos   & 0.609 & 10 \\
% LSTM + $L_2$ & \textbf{0.700} & 10 \\
% \midrule[0.5pt]\bottomrule[1pt]
% \end{tabularx}
% }
% \end{table}
According to the results shown in \autoref{fig:rocs_deep_repr_delta_5} and \autoref{tab:tsb_deep_repr_t}, we can see that, even though the adversarial detectors were trained on different attacks, they displayed high performances in detecting kNN-guided attacks too.
This result has a relevant significance since it means that, despite the different attacks' objectives, adversarial samples share some common behaviours in the inner layers of a deep model.
Moreover, it highlights the generalization capacity of our detection approach. 
Furthermore, we can acknowledged that while the AUC values were very close for the targeted attacks, in the case of untargeted attacks the LSTM performed considerably better than the MLP. 

